Massive Uncoordinated Multiple Access for Beyond 5G

Existing wireless communication systems have been mainly designed to provide substantial gain in terms of data rates. However, 5G and Beyond will depart from this scheme, with the objective not only to provide services with higher data rates. One of the main goals is to support massive machine-type communications (mMTC) in the IoT applications. Supporting massive uplink (UP) communications for devices with sporadic traffic pattern and short-packet size, as it is in many mMTC use cases, is a challenging task, particularly when the control signaling is not negligible in size compared to the payload. Also, channel estimation is challenging for sporadic and short-packet transmission due to the limited number of employed pilots. In this paper, a new UP multiple access (MA) scheme is proposed for mMTC, which can support a large number of uncoordinated IoT devices with short-packet and sporadic traffic. The proposed UP MA scheme removes the overheads associated with the device identifier as well as pilots related to channel estimation. An alternative mechanism for device identification is proposed, where a unique spreading code is dedicated to each IoT device. This unique code is simultaneously used for the spreading purpose and device identification. Two IoT device identification algorithms which employ sparse signal reconstruction methods are proposed to determine the active IoT devices prior to data detection. Specifically, the BIC model order selection method is employed to develop an IoT device identification algorithm for unknown and time-varying probability of device activity. Our proposed MA scheme benefits from a non-coherent multiuser detection algorithm based on machine learning to enable data detection without a priori knowledge on channel state information. The effectiveness of the proposed MA scheme for known and unknown probability of activity is supported by simulation results.

==> WINS-Catechism.tex <==
%----------------------------------------------------------------------------------------%
%                                   W I N S   C a t e c h i s m                              %
%----------------------------------------------------------------------------------------%
\section*{WGroup Research Paper Catechism\footnote{Adapted from George Heilmeier.}} 

\vspace{0.5cm} 

\be\itemsep3ex

\item What is the big picture? What is the problem and why is it hard?
	\bi
	\item[$\diamond$] The Big Picture: \BigPicture
	\item[$\diamond$] The Problem/Difficulty: \ProblemDifficulty
%	\item[$\diamond$] The Difficulty:
	\ei

\item What are the classical approaches? What is the state-of-the-art and what are the deficiencies?
	\bi
	\item[$\diamond$] Classical Approaches: \ClassicApproach
	\item[$\diamond$] The State-of-the-Art and Deficiencies:  \SOADeficiency
	\item[ ] \mysubsubnote{This is where you make a literature review. Articulate the deficiencies and shortcomings of previous work. Provide references (you can use the first three alphabets of the authors' last names and year, similar to the convention in our database).}
	\ei
	
\item What are the fundamental questions relevant to the problem? How answering to these questions can impact the design, architecture, and operation?
	\bi
	\item[$\circ$] \FundamentalQ
	\item[$\circ$] \EnablingA 
	\item[ ] \mysubsubnote{This is where you persuade the reader that these are fundamental questions, and the answers to these questions will have game-changing impacts.}
	\ei	

\item What are the goals of our paper?
	\bi
	\item[$\diamond$] The Goals:
	\item[ ] \mysubsubnote{Describe the goals at a high level; this should correlate with high-level contributions in Question 6.}
	\ei
		\be
		\item[$\circ$] \Goals 
		\ee		
\item What are we advocating; what is the new technical idea; what is our new view; what is our credence? Why we can succeed now? 
	\bi
	\item[$\diamond$] Advocacy, Idea, View, and Credence:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \Advocacy 
		\ee
	\item[$\diamond$] Reasons for Success:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \ReasonSuccess 
		\ee
	\ei

\item What are the high-level contributions of our  paper? What are the key contributions of our paper? 
	\bi
	\item[$\diamond$] High-Level Contributions: \HLContribution
	\item[ ] \mysubsubnote{Describe what we do at a high level; this should address the goal that we set out in Question 4; for example:}
		\be
		\item[$\circ$] In this paper, \ldots
		\ee
	\item[$\diamond$] Key Contributions:
	\item[ ] \mysubsubnote{Provide a bulletized list (usually 3-5 bullets, equal number of lines per bullets); for example:}
		\be
		\item[$\circ$] \KeyContribution
		\ee
	\ei


\item Which are the methodologies (analysis, simulation, experimentation, heterogeneous approach) used in this paper? How is the approach verified; how are the results confirmed?
	\bi
	\item[$\diamond$] The Methodologies:
	\item[$\diamond$] The Verification:
	\ei
	
\item What are the new vision/perspective we provide? What are the lessons learned?
	\bi
	\item[$\diamond$] The New Vision/Perspective: \ConclusiveVision
	\item[$\diamond$] The Lessons Learned/Surprising Results: \ConclusiveLesson
	\ei

\item What is the impact; what are the benefits or merits of the results to a broader community?
	\bi
	\item[$\diamond$] The Impact/Benefit: \Benefit
	\item[ ] \mysubsubnote{Think of strong conclusions for the paper when answering them}
	\ei


\item Where the known results appear in the paper?
	\bi
	\item[$\diamond$] Disclosures:
	\item[ ] \mysubsubnote{Identify where known results appear in the paper (point to specific section numbers before the paper is written; point to specific section, page, line, equation numbers, etc. after the paper is written).}
	\item[$\diamond$] Sources:
	\item[ ] \mysubsubnote{Identify what are the sources (provide reference, section, page, line, equation numbers, etc. of the sources).}
	\ei

\item What are the key references?
\bi
	\item[ ] \mysubsubnote{List the key references that we used to develop this paper (rather than the references for the state-of-the-art).}
\ei

\ee


==> Wgroup-Teaching-Preamble.tex <==
% Greek lowercase letters, sans serif font - by Guido
%
%% =========== Euler ==========
%\DeclareMathAlphabet{\matheur}{U}{eur}{m}{n}
%\SetMathAlphabet{\matheur}{bold}{U}{eur}{b}{n}
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\matheur{#1}\fi%for math sans serif (Euler)
%}
%% =========================
%
% ==== Computer Modern Sans Serif ====
%\DeclareMathAlphabet{\mathsfbr}{OT1}{cmss}{m}{n}%for math sans serif (cmss)
%\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmss}{bx}{n}%for math sans serif (cmss)
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif (cmss)
%}
% =========================

% ==== Computer Modern Bright ====
% Part 1: This is necessary to fix a bug in the .fd file of the font!!!
\DeclareFontFamily{OT1}{cmbr}{\hyphenchar\font45 }
\DeclareFontShape{OT1}{cmbr}{m}{n}{%
  <-9>cmbr8
  <9-10>cmbr9
  <10-17>cmbr10
  <17->cmbr17
}{}
\DeclareFontShape{OT1}{cmbr}{m}{sl}{%
  <-9>cmbrsl8
  <9-10>cmbrsl9
  <10-17>cmbrsl10
  <17->cmbrsl17
}{}
\DeclareFontShape{OT1}{cmbr}{m}{it}{%
  <->ssub*cmbr/m/sl
}{}
\DeclareFontShape{OT1}{cmbr}{b}{n}{%
  <->ssub*cmbr/bx/n
}{}
\DeclareFontShape{OT1}{cmbr}{bx}{n}{%
  <->cmbrbx10
}{}
% Part 2
\DeclareMathAlphabet{\mathsfbr}{OT1}{cmbr}{m}{n}%for math sans serif bright (cmbr)
\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmbr}{b}{n}%for math sans serif bright (cmbr)
\DeclareRobustCommand{\msf}[1]{%
  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif bright (cmbr)
}
% =========================

\makeatletter
\newcommand{\msfgreek}[1]{\csname s\expandafter\@gobble\string#1\endcsname}
\makeatother

% Sans serif greek
\DeclareSymbolFont{sfletters}{U}{eur}{m}{n}\SetSymbolFont{sfletters}{bold}{U}{eur}{b}{n}%for Euler Greek
%\DeclareSymbolFont{sfletters}{FMS}{futm}{m}{n}\SetSymbolFont{sfletters}{bold}{FMS}{futm}{b}{n}%for Euler Greek

\DeclareMathSymbol{\sGamma}{\mathord}{sfletters}{0}
\DeclareMathSymbol{\sDelta}{\mathord}{sfletters}{1}
\DeclareMathSymbol{\sTheta}{\mathord}{sfletters}{2}
\DeclareMathSymbol{\sLambda}{\mathord}{sfletters}{3}
\DeclareMathSymbol{\sXi}{\mathord}{sfletters}{4}
\DeclareMathSymbol{\sPi}{\mathord}{sfletters}{5}
\DeclareMathSymbol{\sSigma}{\mathord}{sfletters}{6}
\DeclareMathSymbol{\sUpsilon}{\mathord}{sfletters}{7}
\DeclareMathSymbol{\sPhi}{\mathord}{sfletters}{8}
\DeclareMathSymbol{\sPsi}{\mathord}{sfletters}{9}
\DeclareMathSymbol{\sOmega}{\mathord}{sfletters}{10}
\DeclareMathSymbol{\salpha}{\mathord}{sfletters}{"0B}
\DeclareMathSymbol{\sbeta}{\mathord}{sfletters}{"0C}
\DeclareMathSymbol{\sgamma}{\mathord}{sfletters}{"0D}
\DeclareMathSymbol{\sdelta}{\mathord}{sfletters}{"0E}
\DeclareMathSymbol{\sepsilon}{\mathord}{sfletters}{"0F}
\DeclareMathSymbol{\szeta}{\mathord}{sfletters}{"10}
\DeclareMathSymbol{\seta}{\mathord}{sfletters}{"11}
\DeclareMathSymbol{\stheta}{\mathord}{sfletters}{"12}
\DeclareMathSymbol{\siota}{\mathord}{sfletters}{"13}
\DeclareMathSymbol{\skappa}{\mathord}{sfletters}{"14}
\DeclareMathSymbol{\slambda}{\mathord}{sfletters}{"15}
\DeclareMathSymbol{\smu}{\mathord}{sfletters}{"16}
\DeclareMathSymbol{\snu}{\mathord}{sfletters}{"17}
\DeclareMathSymbol{\sxi}{\mathord}{sfletters}{"18}
\DeclareMathSymbol{\spi}{\mathord}{sfletters}{"19}
\DeclareMathSymbol{\srho}{\mathord}{sfletters}{"1A}
\DeclareMathSymbol{\ssigma}{\mathord}{sfletters}{"1B}
\DeclareMathSymbol{\stau}{\mathord}{sfletters}{"1C}
\DeclareMathSymbol{\supsilon}{\mathord}{sfletters}{"1D}
\DeclareMathSymbol{\sphi}{\mathord}{sfletters}{"1E}
\DeclareMathSymbol{\schi}{\mathord}{sfletters}{"1F}
\DeclareMathSymbol{\spsi}{\mathord}{sfletters}{"20}
\DeclareMathSymbol{\somega}{\mathord}{sfletters}{"21}
\DeclareMathSymbol{\svarepsilon}{\mathord}{sfletters}{"22}
\DeclareMathSymbol{\svartheta}{\mathord}{sfletters}{"23}
\DeclareMathSymbol{\svarpi}{\mathord}{sfletters}{"24}
\DeclareMathSymbol{\svarrho}{\mathord}{sfletters}{"25}
\DeclareMathSymbol{\svarsigma}{\mathord}{sfletters}{"26}
\DeclareMathSymbol{\svarphi}{\mathord}{sfletters}{"27}

\DeclareRobustCommand{\mcal}[1]{%
  \ifcat\noexpand#1\relax\mathnormal{#1}\else\cal{#1}\fi
}
%-------------------------
% Math symbol
%-------------------------
\newcommand{\rv}[1]{\MakeLowercase{\msf{#1}}}  
\newcommand{\RV}[1]{\boldsymbol{\MakeLowercase{\msf{#1}}}}
\newcommand{\RM}[1]{\boldsymbol{\MakeUppercase{\msf{#1}}}}
\newcommand{\RS}[1]{\MakeUppercase{\msf{#1}}}

\newcommand{\V}[1]{\boldsymbol{\MakeLowercase{#1}}}
\newcommand{\M}[1]{\boldsymbol{\MakeUppercase{#1}}}
\newcommand{\Set}[1]{\MakeUppercase{\mcal{#1}}}

